GLAMpoints: Greedily Learned Accurate Match points

We introduce a novel CNN-based feature point detector - GLAMpoints - learned in a semi-supervised manner. Our detector extracts repeatable, stable interest points with a dense coverage, specifically designed to maximize the correct matching in a specific domain, which is in contrast to conventional techniques that optimize indirect metrics. In this paper, we apply our method on challenging retinal slitlamp images, for which classical detectors yield unsatisfactory results due to low image quality and insufficient amount of low-level features. We show that GLAMpoints significantly outperforms classical detectors as well as state-of-the-art CNN-based methods in matching and registration quality for retinal images. Our method can also be extended to other domains, such as natural images. Training code and model weights are available at https://github.com/PruneTruong/GLAMpoints_pytorch.

==> rebuttal.tex <==

We would like to thank all the reviewers for their comments, which we address below.
In the paper and the following, any reference to SIFT descriptor is root-SIFT. 
%------------------------------------------------------------------------
\par \textbf{R1: Generalization of GLAMpoints.}
We used SIFT descriptor for GLAMpoints due to its superior performance for retinal images [1], but the training procedure can be used in conjunction with other descriptors. We ran experiments using GLAMpoints trained with ORB and BRISK descriptors, improving on the original detectors (Table \ref{tab:comparisons} top).
%------------------------------------------------------------------------
\par \textbf{R2: Root-SIFT as a descriptor for other methods.}
We used the descriptors that were developed/trained jointly with the detector and can be considered as optimal. In [44] the combination of the LIFT detector and the SIFT descriptor performed worse compared to the LIFT detector/descriptor and the importance of using jointly optimized detector/descriptor pairs is further stressed in [31]. We present the evaluation of other detectors with root-SIFT descriptors (Table~ \ref{tab:comparisons} middle).  SIFT does not improve the result compared to the original descriptor.
%------------------------------------------------------------------------
\par \textbf{R3: Generalization to natural images.}
The main focus of this paper were retinal images, which prove to be challenging for SOTA approaches. Even though LF-NET generalized well to retinal images w.r.t. the metrics it was optimized for (\ie repeatability), Table 2 of the paper shows that the final registration accuracy of LF-NET is significantly lower than our method. As R3 pointed out, generalization from biomedical to natural images is harder than vice versa. We believe that training our method on natural images could improve the results in that domain further. We will emphasize that GLAMpoints outperform classical detectors in the domain of \textit{retinal} images, with a possible extension to natural images. 

%------------------------------------------------------------------------
\par \textbf{R2, R3: Uniform distribution of GLAMpoints.} To verify that the performance gain does not come solely from the uniform spread of the points we computed the success rate for keypoints in a random, uniformly distributed grid  (Table~\ref{tab:comparisons} bottom). The number of detected keypoints depends only on the NMS width. 
%------------------------------------------------------------------------

\par \textbf{R2, R3: Relation to Reinforcement Learning} As R2 and R3 have pointed out, our method does not follow the common definition of RL as a Markov Decision Process. We used the idea of delayed reward (registration accuracy), which relates to RL. We will clarify this in the final version.

%------------------------------------------------------------------------

\par \textbf{R1,R3: Experimental setup.}
    \textbf{Training}: final results were obtained applying a single model trained on the full slit lamp training set (raw images). We ensured that images in the train and test sets correspond to different patients. $256 \times 256$ patches were randomly cropped to speed up the \textit{training} processes.
    \textbf{Homographies}: to obtain the ground-truth homographies for the slit lamp, we followed common strategies~([4]). As slit lamp and fundus images capture small part of the retina, the planar assumption can be applied~[2][3]. 
    \textbf{FIRE}: was only used to \texit{test} the model trained on $slit lamp$ images. The testing image pairs thus correspond to the ones described in [22]. They were down-scaled to 15\% to match the resolution of the slit lamp images. We did not use the retina masks to filter out border keypoints as generally they were not matched and they did not contribute to the final registration. 
    \textbf{Metrics}: the registration \textit{failed} if not enough keypoints or matches were found for a homography (minimum 4), or if it contains a flip or the estimated scale component is greater than 4 or less than 0.1. Different thresholds for acceptable registrations are used for slit lamp 
    §
    and $FIRE$ datasets - to compare with the same threshold see Table~\ref{tab:FIRE_threshold}.
    \textbf{Natural images}: due to space constraints and the focus on retinal images, we included experiment details on natural images in the supplementary material. We used the homographies provided by the authors of the datasets and the same thresholds as for slit lamp dataset.
The above-mentioned experimental details will be added in the final version of the paper.


%------------------------------------------------------------------------
\par \textbf{R1,R3: Relevant literature} In the final version of the paper we will add the discussion of the suggested literature and add the missing information in the current citations.

\begin{table}[t]

\centering
\caption{Success rates on slit lamp images, with GLAMpoints detector trained on the descriptor in parenthesis.}
\vspace{-4mm}
\label{tab:comparisons}
\resizebox{0.40\textwidth}{!}{%
\begin{tabular}{lllll@{}}
\toprule
Detector & Descriptor  & Failed {[}\%{]} & Inaccurate {[}\%{]} & Acceptable {[}\%{]} \\ \midrule
ORB & ORB & 9.71 & 83.01 & 7.28 \\
GLAMpoints (ORB) & ORB & 0.0 & 88.35 & \textbf{11.65} \\
BRISK & BRISK & 16.99 & 66.02 & 16.99 \\
GLAMpoints (BRISK) & BRISK & 1.94 & 75.73 & \textbf{22.33}
\\ \midrule\midrule
SIFT & SIFT & 1.94 & 47.75 & 50.49 \\
KAZE & KAZE  & 1.46            & 54.85                          & 43.69  \\
KAZE & SIFT  & 4.37               & 57.28                 & 38.35   \\
SuperPoint & Superpoint & 7.77            & 51.46                          & 40.78\\
SuperPoint & SIFT & 6.80  & 54.37                 & 38.83  \\
LF-NET & LF-NET & 0.0                & 36.89                 & 63.11       \\
LF-NET & SIFT & 0.0                & 40.29                 & 59.71 \\
GLAMpoints (SIFT) & SIFT  & 0.0             & 31.55                          & 68.45
\\\midrule\midrule
Random grid  & SIFT  & 0.0    & 62.62                 & 37.38  \\
\bottomrule
\end{tabular}%
}
\label{tab:improved_detector}
\vspace{-3mm}
\end{table}

\begin{table}[t]
\centering
\caption{Success rates (\%) for each detector on \textit{FIRE} dataset with bigger threshold ("acceptable" registrations  when $MEE<10$ and $MAE<30$).}
\vspace{-4mm}
\label{tab:success-rate-FIRE}
\resizebox{0.40\textwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
                                  & Failed {[}\%{]} & Inaccurate {[}\%{]} & Acceptable {[}\%{]} \\ \midrule
SIFT                              & 2.24 & 36.57                 & 61.19                 \\
KAZE                              & 14.18 & 58.21    & 27.61                 \\
SuperPoint                        & 0.0                & 13.43                 & 86.57     \\
LIFT                              & 0.0                & 10.45                 & 89.55           \\
LF-NET                            & 0.0 & 38.06 & 61.94 \\
GLAMpoints (OURS)                 & 0.0                & 5.22    & \textbf{94.78}        \\ \bottomrule
\end{tabular}%
}
\vspace{-7mm}
\label{tab:FIRE_threshold}
\end{table}



%------------------------------------------------------------------------
\par \textbf{References}
\newline [1] C. Hernandez-Matas, et al., An Experimental Evaluation of the Accuracy of Keypoints-based Retinal Image Registration, EMBC, 2017
\newline [2] P.C. Cattin., et al., Retina Mosaicing Using Local Features. MICCAI, 2006
\newline [3] L. Giancardo, et al., Textureless Macula Swelling Detection With Multiple Retinal Fundus Images. IEEE TBME, 2011
%\newline [4] R. Hartley and A. Zisserman, Multiple View Geometry in Computer %Vision, 2003
\newline [4] J. Chen, et al. A Partial Intensity Invariant Feature Descriptor for Multimodal Retinal Image Registration.IEEE TBME 2010
\newline [5] G. Wang, et al., Robust point matching method for multimodal retinal image registration. BSPC 2015
